SGPMIL: Sparse Gaussian Process Multiple Instance Learning

Multiple Instance Learning (MIL) offers a natural solution for settings where only coarse, bag-level labels are available, without having access to instance-level annotations. This is usually the case in digital pathology, which consists of gigapixel-sized images. While deterministic attention-based MIL approaches achieve strong bag-level performance, they often overlook the uncertainty inherent in instance relevance. In this paper, we address the lack of uncertainty quantification in instance-level attention scores by introducing SGPMIL, a new probabilistic attention-based MIL framework grounded in Sparse Gaussian Processes (SGP). By learning a posterior distribution over attention scores, SGPMIL enables principled uncertainty estimation, resulting in more reliable and calibrated instance relevance maps. Our approach not only preserves competitive bag-level performance but also significantly improves the quality and interpretability of instance-level predictions under uncertainty. SGPMIL extends prior work by introducing feature scaling in the SGP predictive mean function, leading to faster training, improved efficiency, and enhanced instance-level performance. Extensive experiments on multiple well-established digital pathology datasets highlight the effectiveness of our approach across both bag- and instance-level evaluations. Our code is available at https://github.com/mandlos/SGPMIL.

==> Supplementary_stuff/inducing_points_ablations.tex <==

    \centering
        \begin{tabular}{lcccccc}
        \toprule
        & \multicolumn{3}{c}{WSI} & \multicolumn{3}{c}{INSTANCE}\\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        \midrule
        $U$ & ACC & AUC & ACE & ACC & AUC & ACE \\
        \midrule
        $16$ & $.971_{.016}$ & $.977_{.020}$ & $.045_{.022}$ & $\underline{.893}$ & $.963$ & $.271$ \\
        
        $32$ & $\underline{.979_{.010}}$ & $\underline{.985_{.005}}$ & $\underline{.026_{.010}}$ & $.880$ & $\underline{.970}$ & $\mathbf{.046}$ \\
        
        $64$ & $.964_{.013}$ & $.981_{.009}$ & $.041_{.016}$ & $.832$ & $.910$ & $.210$\\
        
        $80$ & $\mathbf{.980_{.007}}$ & $\mathbf{.986_{.005}}$ & $\mathbf{.021_{.005}}$ & $\mathbf{.914}$ & $\mathbf{.973}$ & $\underline{.051}$\\
        \bottomrule
        \end{tabular}
    \caption{Performance of SGPMIL on the CAMELYON16 dataset for varying numbers of inducing points ($U$). Slide-level metrics (WSI) and instance-level metrics are reported. Instance-level accuracy (ACC) is computed using the optimal binarization threshold for each model, following the evaluation protocol introduced in BayesMIL.}
    \label{tab:inducing_points_ablations_sgpmil}


==> Supplementary_stuff/train_test_times.tex <==
\centering
\begin{tabular}{lcc}
\toprule
Model & Training Time (h) & Inference Time (s) \\
\midrule
ABMIL & 5.5 & 0.8 \\
CLAM & 7.0 & 0.9 \\
TransMIL & 13.4 & 1.2 \\
DGRMIL & 16.7 & 1.5 \\
BayesMIL & 9.5 & 1.1 \\
AGP & 31.0 & 6.0 \\
SGPMIL & 9.0 & 1.0 \\
\bottomrule
\end{tabular}
\label{tab:times}
\caption{fjdkl;fasldkfj}

==> sections/7_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
